Bifurcation and multiple states in plane Couette flow with spanwise rotation

We present a derivation that begins with the Navier--Stokes equation and ends with a prediction of multiple statistically stable states identical to those observed in a spanwise rotating plane Couette flow. This derivation is able to explain the presence of multiple states in fully developed turbulence and the selection of one state over the other by differently sized computational domains and different initial conditions. According to the present derivation, two and only two statistically stable states are possible in an infinitely large plane Couette flow with spanwise rotation, and that multiple states are not possible at very slow or very rapid rotation speeds. We also show the existence of limit cycles near statistically stable states.

==> macros.tex <==
%\usepackage[dvips]{graphicx,color}
\usepackage{graphicx,color}
\usepackage{amssymb,latexsym}
\usepackage{url}

% For units of measure
%\newcommand\dynpercm{\nobreak\mbox{$\;$dynes\,cm$^{-1}$}}
%\newcommand\cmpermin{\nobreak\mbox{$\;$cm\,min$^{-1}$}}

% Various bold symbols
%\providecommand\bnabla{\boldsymbol{\nabla}}
%\providecommand\bcdot{\boldsymbol{\cdot}}
%\newcommand\biS{\boldsymbol{S}}
%\newcommand\etb{\boldsymbol{\eta}}
%\newcommand\bomega{\boldsymbol{\omega}}

% For multiletter symbols
%\newcommand\Real{\mbox{Re}} % cf plain TeX's \Re and Reynolds number
%\newcommand\Imag{\mbox{Im}} % cf plain TeX's \Im
%\newcommand\Rey{\mbox{\textit{Re}}}  % Reynolds number
%\newcommand\Pran{\mbox{\textit{Pr}}} % Prandtl number, cf TeX's \Pr product
%\newcommand\Pen{\mbox{\textit{Pe}}}  % Peclet number
%\newcommand\Ai{\mbox{Ai}}            % Airy function
%\newcommand\Bi{\mbox{Bi}}            % Airy function

% -----------------------  colores ----------------------------
%\def\azul{\textcolor{blue}}
%\def\negro{\textcolor{black}}
%\def\rojo{\textcolor{red}}
%\def\magenta{\textcolor{magenta}}
%\def\verde{\textcolor{green}}

%%%%%%%%%%%% etiquetas y leyendas
\newcommand{\mylab}[3]{\raisebox{#2}[0mm][0mm]{%
\makebox[0mm][l]{\hspace*{#1}\textbf{#3}}}}
\def\spacce#1{\hskip #1pt}
\def\drawline#1#2{\raise 2.5pt\vbox{\hrule width #1pt height #2pt}}
\def\solid{\drawline{24}{.5}\nobreak}
\def\solidthick{\drawline{24}{1.5}\nobreak}
\def\bdashli{\hbox{\drawline{5}{.5}\spacce{2}}}
\def\bdash{\hbox{\drawline{5.8}{.5}\spacce{2}}}
\def\bdashort{\hbox{\drawline{3.5}{.5}\spacce{1}}}
\def\bdashthick{\hbox{\drawline{1}{1.5}\spacce{2}}}
\def\dashed{\bdash\bdash\bdash\nobreak}
\def\dashdash{\bdashort\bdashort\spacce{3}\bdashort\bdashort\nobreak}
\def\dashedthick{\bdashthick\bdashthick\bdashthick\bdashthick\nobreak}
\def\bdot{\hbox{\drawline{1}{.5}\spacce{2}}}
\def\bdotthick{\hbox{\drawline{1}{1.5}\spacce{2}}}
\def\dotted{\hbox{\leaders\bdot\hskip 24pt}\nobreak}
\def\dottedthick{\hbox{\leaders\bdotthick\hskip 24pt}\nobreak}
\def\dchndot{\hbox%
{\drawline{4.6}{.5}\spacce{2}\drawline{1}{.5}\spacce{4.6}\drawline{4.6}{.5}\spacce{2}\drawline{1}{.5}}\nobreak }
\def\chndot{\hbox%
{\drawline{4.6}{.5}\spacce{2}\drawline{1}{.5}\spacce{2}\drawline{4.6}{.5}\spacce{2}\drawline{1}{.5}\spacce{2}\drawline{4.6}{.5}}\nobreak }
\def\circle{$\circ$\nobreak }
\def\linecir{\hbox%
{\drawline{8}{.5}\spacce{2}\circle\spacce{2}\drawline{8}{.5}}\nobreak}
\def\trian{\raise 1.25pt\hbox{$\scriptstyle\triangle$}\nobreak}
\def\linetri{\hbox%
{\drawline{8}{.5}\spacce{2}\trian\drawline{8}{.5}}\nobreak}
\def\dtrian{\raise 1.25pt\hbox%
{$\scriptscriptstyle\bigtriangledown$}\nobreak}
\def\linedtrian{\hbox%
{\drawline{8}{.5}\spacce{2}\dtrian\drawline{8}{.5}}\nobreak}
\def\squar{\raise 1.25pt\hbox{$\scriptstyle\Box$}\nobreak}
\def\linesquar{\hbox%
{\drawline{8}{.5}\spacce{2}\squar\drawline{8}{.5}}\nobreak}
\def\diamon{\raise 1.25pt\hbox{$\scriptstyle\diamond$}\nobreak}
%\def\soliddiamon{\raise 1.25pt\hbox{$\scriptstyle\vardiamond$}\nobreak}
\def\linediam{\hbox%
{\drawline{8}{.5}\spacce{2}\diamon\drawline{8}{.5}}\nobreak}
\def\solidtrian{$\blacktriangle$\nobreak}
\def\soliddtrian{$\blacktriangledown$\nobreak}
\def\linesolidtrian{\hbox%
{\drawline{8}{.5}\spacce{2}\solidtrian\drawline{8}{.5}}\nobreak}
\def\solidsquar{$\blacksquare$\nobreak}
\def\linesolidsquar{\hbox%
{\drawline{8}{.5}\spacce{2}\solidsquar\drawline{8}{.5}}\nobreak}
\def\solidcircle{$\bullet$\nobreak}
\def\linestar{\hbox%
{\drawline{8}{.5}\spacce{2}$*$\spacce{2}\drawline{8}{.5}}\nobreak}
\def\dottrian{\bdot\bdot\bdot\trian\spacce{2}\bdot\bdot\bdot}
\def\dotdtrian{\bdot\bdot\bdot\dtrian\spacce{2}\bdot\bdot\bdot}
\def\dotsolidtrian{\bdot\bdot\bdot\solidtrian\spacce{2}\bdot\bdot\bdot}
\def\dotsquar{\bdot\bdot\bdot\squar\spacce{2}\bdot\bdot\bdot}
\def\dotsolidcircle{\bdot\bdot\bdot\solidcircle\spacce{2}\bdot\bdot\bdot}
\def\dotsolidsquar{\bdot\bdot\bdot\solidsquar\spacce{2}\bdot\bdot\bdot}
\def\dashtrian{\bdashli\bdashli\trian\spacce{2}\bdashli\bdashli}
\def\dashsolidtrian{\bdashli\bdashli\solidtrian\spacce{2}\bdashli\bdashli}
\def\dashsquar{\bdashli\bdashli\squar\spacce{2}\bdashli\bdashli}
\def\dashsolidsquar{\bdashli\bdashli\solidsquar\spacce{2}\bdashli\bdashli}
\def\linetimes{\hbox%
{\drawline{8}{.5}\spacce{2}$\times$\spacce{2}\drawline{8}{.5}}\nobreak}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% matematicas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% matematicas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% matematicas
\def\dd{{\, \rm{d}}}
\def\bra{\langle}
\def\ket{\rangle}
\def\p{\partial}
\def\ra{\rightarrow}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\la{\label}
%
\def\utau{u_\tau}
\def\retau{Re_\tau}
%
\def\aaa{{\it a}}
\def\bbb{{\it b}}
\def\ccc{{\it c}}
\def\ddd{{\it d}}
\def\eee{{\it e}}
\def\fff{{\it f}}
\def\ggg{{\it g}}
\def\hhh{{\it h}}
\def\iii{{\it i}}
\def\jjj{{\it j}}
%
\newcommand\ab{{\it ab}\ }
\newcommand\bc{{\it bc}\ }
\newcommand\cd{{\it cd}\ }
\newcommand\ad{{\it ad}\ }
%%%%%%%%5% citas exoticas
%\def\citalajim03{Del \'Alamo \& Jim\'enez (2003)}
% macros miscelaneas
\newcommand\ie{i.e.\ }

%%% PARA EL CURRICULUM

%\newenvironment{history}{\begin{list}{}{\setlength{\leftmargin}{2.4cm}
%\setlength{\labelwidth}{2.4cm} \setlength{\labelsep}{0cm}}}{\end{list}}

%\newenvironment{history2}{\begin{list}{}{\setlength{\leftmargin}{3.5cm}
%\setlength{\labelwidth}{3.5cm} \setlength{\labelsep}{0cm}}}{\end{list}}

%\newenvironment{hitos}{\begin{list}{$\bullet$
%\hfill}{\setlength{\leftmargin}{0.4cm} \setlength{\labelwidth}{0.4cm}
%\setlength{\labelsep}{0cm}}}{\end{list}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%               FIN MACROS MIAs                    %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

